MSDN: Mutually Semantic Distillation Network for Zero-Shot Learning

The key challenge of zero-shot learning (ZSL) is how to infer the latent semantic knowledge between visual and attribute features on seen classes, and thus achieving a desirable knowledge transfer to unseen classes. Prior works either simply align the global features of an image with its associated class semantic vector or utilize unidirectional attention to learn the limited latent semantic representations, which could not effectively discover the intrinsic semantic knowledge e.g., attribute semantics) between visual and attribute features. To solve the above dilemma, we propose a Mutually Semantic Distillation Network (MSDN), which progressively distills the intrinsic semantic representations between visual and attribute features for ZSL. MSDN incorporates an attribute$\rightarrow$visual attention sub-net that learns attribute-based visual features, and a visual$\rightarrow$attribute attention sub-net that learns visual-based attribute features. By further introducing a semantic distillation loss, the two mutual attention sub-nets are capable of learning collaboratively and teaching each other throughout the training process. The proposed MSDN yields significant improvements over the strong baselines, leading to new state-of-the-art performances on three popular challenging benchmarks, i.e., CUB, SUN, and AWA2. Our codes have been available at: \url{https://github.com/shiming-chen/MSDN}.

==> dashrule/README <==
               +--------------------------------------+
               |   DASHRULE: Dashed rules in LaTeX    |
               | By Scott Pakin, scott+dash@pakin.org |
               +--------------------------------------+


Description
-----------

The dashrule package makes it easy to draw a huge variety of dashed
rules (i.e., lines) in LaTeX.  dashrule provides a command,
\hdashrule, which is a cross between LaTeX's \rule and PostScript's
setdash command.  \hdashrule draws horizontally dashed rules using the
same syntax as \rule, but with an additional, setdash-like parameter
that specifies the pattern of dash segments and the space between
those segments.  Because dashrule's rules are constructed internally
using \rule (as opposed to, e.g., PostScript \specials) they are fully
compatible with every LaTeX back-end processor.


Installation
------------

There's nothing special about building dashrule:

    latex dashrule.ins     <== Generate dashrule.sty
    latex dashrule.dtx     <== Produce the documentation (dashrule.dvi)
    makeindex -s gind.ist dashrule    <== Generate an index
    latex dashrule.dtx     <== Incorporate the index into the document

If you're new to this, see
http://www.tex.ac.uk/cgi-bin/texfaq2html?label=instpackages for more
information on installing packages.


Copyright and license
---------------------

Copyright (C) 2013 Scott Pakin, scott+dash@pakin.org

This package may be distributed and/or modified under the conditions
of the LaTeX Project Public License, either version 1.3c of this
license or (at your option) any later version.  The latest version of
this license is in:

    http://www.latex-project.org/lppl.txt

and version 1.3c or later is part of all distributions of LaTeX version
2006/05/20 or later.

